Measurement-Based Modeling of Short Range Terahertz Channels and Their Capacity Analysis

In this work, extensive propagation characteristics of short range 240 to 300 GHz terahertz (THz) channels are mapped based on a measurement campaign conducted utilizing a novel, task specific measurement system. The measurement system allows collecting measurements from different distances and orientations in a very fine grained resolution, which is a particular issue in achieving realistic THz channel estimation. After the accurate measurement results are obtained, they are investigated in terms of channel impulse and channel frequency response. Furthermore, the fading channel amplitude histograms are modeled with the Gamma mixture model (GMM). The expectation-maximization (EM) algorithm is utilized to determine the corresponding mixture parameters. Also, to demonstrate the flexibility of the GMM, the Dirichlet process Gamma mixture model (DPGMM) is utilized in cases where the EM algorithm fails to represent histograms. Moreover, the suitability of the GMM is evaluated utilizing Kolmogorov Smirnov tests. Results verify that the GMMs can simulate the fading channel of micro-scale THz wireless communication in a realistic way, providing important implications regarding the achievable capacity in these channels. Finally, the average channel capacity of each link is evaluated using the probability density function of GMMs to gain deeper insight into the potential of micro-scale THz communications.

==> some_notes.tex <==
% The demand for wireless data is increasing rapidly due to the proliferation of smartphones, tablets, and other connected devices. This increase in demand is putting pressure on existing frequency bands, which are becoming increasingly congested. As a result, there is a need for additional spectrum to support the growing demand for wireless data.

% However, there are challenges to employing the THz spectrum for communication, such as significant atmospheric gas absorption in particular frequencies, which limits the communication range.
% As a result, the THz band exhibits unique channel characteristics compared to other commonly operated frequency spectrums; even different THz windows can have distinctive channel properties.
% % Due to these reasons, the THz frequency band should be modeled more carefully.
% To understand these difficulties and model the THz band particularities, several measurement-based works have been done \cite{ekti2017statistical,kim2014statistical,tekbiyik2019statistical,nguyen2021large,chen2021channel,fu2020modeling,kim2016characterization,eckhardt2019measurements} to characterize large-scale fading characteristics.
% In~\cite{ekti2017statistical}, frequency-dependent path loss parameters of the THz channels are measured for LOS conditions. 
% The single slop path loss model with shadow fading parameters is derived for the desktop channel between 300 and 320 GHz in~\cite{kim2014statistical}.  
% The two-slope path loss model for the short-range THz propagation is given in~\cite{tekbiyik2019statistical}, which demonstrates the joint effect of the transmitter-receiver separation and the frequency on the received power. The large-scale parameters of the spatio-temporal channel for 140 GHz at the shopping mall and airport hall are investigated in \cite{nguyen2021large}.
% An indoor communication hybrid cluster-based channel modeling is proposed for 130 GHz - 143 GHz in \cite{chen2021channel} by combining ray-tracing and statistical methods.
% Furthermore, the characterization of chip-to-chip, computer motherboard, and data center channel characterization is conducted in \cite{fu2020modeling,kim2016characterization,eckhardt2019measurements} respectively.  

% To gain a deeper understanding of these challenges and model the THz band's peculiarities, researchers have conducted various measurement-based studies \cite{ekti2017statistical,kim2014statistical,tekbiyik2019statistical,nguyen2021large,chen2021channel,fu2020modeling,kim2016characterization,eckhardt2019measurements} to characterize large-scale fading characteristics and the factors affecting it.


% Despite the vast potential of the THz spectrum for communication, it presents several challenges, such as the absorption of signals by atmospheric gases at specific frequencies, which can limit communication range. Due to this, the THz band has unique channel characteristics compared to other commonly used frequency spectrums, and even different THz windows can have dissimilar properties. To overcome these challenges and understand the intricacies of the THz band, researchers have conducted a number of measurement-based studies [citations] to investigate the large-scale fading characteristics. These studies [citations] have explored different scenarios such as LOS conditions, short-range and long-range communication, indoor and outdoor environments, and diverse situations like shopping malls, airport halls, and data centers, to name a few. The findings from these studies have provided useful insights and proposed models that can help in modeling and understanding the unique characteristics of the THz band and pave the way for its effective utilization.

% The THz spectrum holds great promise for communication, but its use is hindered by challenges such as the significant absorption of signals by atmospheric gases at certain frequencies, which limits the communication range. This results in unique channel characteristics in the THz band compared to other frequency spectrums commonly used, and even different THz windows can have distinct properties. To gain a deeper understanding of these challenges and model the THz band's peculiarities, researchers have conducted various measurement-based studies [citations] to characterize large-scale fading characteristics and the factors affecting it, such as LOS condition, Distance, Indoor and Outdoor scenarios, and diverse environments like shopping malls and airport halls. These studies have provided a detailed characterization of THz channels and proposed models that can help in modeling and understanding the unique characteristics of the THz band and pave the way for its successful deployment in diverse communication application scenarios.


% In addition, \cite{papasotiriou2021new}, measurements that were conducted on a shopping mall, airport, and a university and suitability of the $\alpha-\mu$ distribution is investigated for characterizing the fading.


% % Even though there is a lot of work put forward  still,  channel characterizations are required for different THz band communication applications. 
% Channel characterizations are still required for various THz band communication applications in order to develop reliable devices.
% Also, the majority of channel measurement studies consider the bandwidth up to 20 GHz. However, when the future THz communication applications are realized, it is anticipated that higher bandwidths will be utilized in practice.  
% Motivated by these, a scenario-specific measurement setup was developed, which allows for taking the measurements from various distances and misalignments to analyze the fading for the micro-scale communication application in the sub-THz channel over 60 GHz bandwidth accurately. 
% High-speed wireless connections between personal mobile terminals, PC/kiosk/cloud servers, and wireless nanosensor communications \cite{akyildiz2010electromagnetic} 
%  can be given as examples of micro-scale communication applications.
% The measurements taken in various settings between 240 GHz and 300 GHz are analyzed in terms of channel impulse response and channel frequency response.
% Also, the suitability of the Gamma mixtures is investigated to model the received power of the measurements. 
% , the capacity of each link is evaluated both numerically and analytically.




% we can gain a deeper understanding of the capacity of these devices and pave the way for their optimal use.


% "To ensure the reliability of THz band communication technology, it is crucial to have a deep understanding of the channels through which the signals will be transmitted. This is achieved through channel characterization. While some measurement studies have been conducted, they typically focus on bandwidths of 20 GHz or less. However, as THz communication technology progresses, it is expected that higher bandwidths will be needed in the future. To prepare for this, a special measurement setup was designed to accurately measure the sub-THz channel over a bandwidth of 60 GHz at various distances and angles, particularly for micro-scale communication applications such as high-speed wireless connections between personal mobile terminals, PC/kiosk/cloud servers, and wireless nanosensor communications. The measurements taken in various settings between 240 and 300 GHz will be analyzed in terms of channel impulse response and frequency response. Additionally, the suitability of using Gamma mixture models to model received power will be investigated, and with this information, the capacity of each link will be evaluated through both numerical and analytical methods."

% To ensure the successful implementation of THz communication technology, it is crucial that we understand how these devices will perform in a range of real-world environments. While previous research has largely focused on THz channels with bandwidths of 20 GHz or less, it is likely that future applications will require higher bandwidths. To address this gap in knowledge, a specialized measurement setup was created to study the performance of micro-scale THz communication devices operating at bandwidths of up to 60 GHz. This setup allows for testing under a variety of distances and misalignment conditions, providing insight into how these devices will perform in real-world scenarios, including high-speed wireless connections between personal mobile devices and servers, as well as wireless communications between nanosensors. By analyzing the channel impulse response and frequency response in the sub-THz range between 240 and 300 GHz, and using Gamma mixture models to evaluate received power, we can more fully understand the capacity and limitations of these devices and pave the way for their successful deployment.

% To make sure THz communication devices can deliver as expected, it's essential to understand how they perform under a variety of real-world conditions. Despite existing research, the majority of studies of THz channels have concentrated on bandwidths no greater than 20 GHz, but the potential for future applications to utilize higher bandwidths has motivated a new approach. Researchers have crafted a custom measurement setup to investigate the performance of micro-scale THz communication devices which operate on bandwidths as high as 60 GHz. This setup allows for testing at different distances and orientations, providing valuable data about how these devices will function in actual scenarios like quick wireless connections between mobile devices, servers, and nanosensors. Through analyzing the channel impulse response and frequency response in the sub-THz range, 240-300 GHz, and utilizing Gamma mixtures to model received power, we can gain a deeper understanding of the capacity of these devices and pave the way for their optimal use.

% Developing dependable communication devices for the THz band requires an understanding of how these devices will behave in a variety of real-world situations. However, most research done on THz channels has focused on bandwidths of 20 GHz or less. To tackle this issue, a unique measurement setup was created specifically to study the performance of micro-scale THz communication devices that operate at bandwidths of up to 60 GHz. This setup enables testing under different distances and misalignment scenarios, providing valuable information on how these devices will function in actual micro-scale communication applications such as high-speed wireless connections between personal mobile devices and servers or wireless communications between nanosensors. By analyzing the channel impulse response and frequency response within the sub-THz range of 240 to 300 GHz and using Gamma mixture models to evaluate received power, we can develop a better understanding of the capacity and capabilities of these devices, paving the way for their successful deployment.

% To build communication devices that perform reliably in the THz band, researchers must examine how they operate under a variety of real-world conditions. Though most studies in this field focus on bandwidths up to 20 GHz, it's expected that future applications will require higher bandwidths. To address this gap in knowledge, scientists have developed a specialized measurement setup to study the performance of micro-scale THz communication devices that operate at bandwidths up to 60 GHz. This setup can be adjusted to test under various distances and misalignment conditions, providing crucial information about how these devices will perform in real-world situations such as high-speed wireless connections between personal mobile devices, servers, and wireless communications between nanosensors. By analyzing the channel impulse response and frequency response within the sub-THz range of 240 to 300 GHz, and using Gamma mixture models to evaluate received power, researchers can gain a deeper understanding of the capacity and capabilities of these devices, paving the way for their successful deployment.

% Motivated by these, to characterize and model the fading in the sub-THz channel accurately, a scenario-specific measurement setup  was developed that allows taking the measurements from various distances and misalignments. 
% The measurement setup can cover micro-scale communication application \cite{akyildiz2010electromagnetic} scenarios like high-speed wireless connections between personal mobile terminals, PC/kiosk/cloud servers, and wireless nanosensor communications.
% The measurements are analyzed in terms of channel impulse response and channel frequency response to validate.   
% and assessed the modeling of the short-range LoS sub-THz band channel. 
 % One important thing to mention, due to the short wavelengths of THz frequencies, smaller antennas will be utilized, which will also result in an expansion of communication applications in next-generation communication systems. One such application area is the microscale communications\cite{he2017stochastic}. Microscale communication includes high-speed wireless connections between personal mobile terminals, PC/kiosk/cloud servers, and wireless nanosensor communications, which link tiny devices across considerably shorter distances \cite{akyildiz2010electromagnetic}.

% However, there are challenges with using the THz frequency band for communication, such as high absorption in specific frequencies due to atmospheric gases. Thus THz band has distinct channel characteristics than other commonly utilized frequency bands. Even various THz sub-bands have different channel characteristics.


% However, there are challenges with using the THz frequency band for communication, such as high absorption by atmospheric gases, which can limit its range.
% Because of these issues, the THz band has distinct channel characteristics than other commonly utilized frequency bands. Even various THz sub-bands have different channel characteristics.


% One potential solution is to make use terahertz (THz) frequency band, which offers very wide bandwidth and could potentially support very high data rates. However, there are also challenges associated with using the THz frequency band for communication, such as the high absorption of THz waves by atmospheric gases, which can limit the range of THz communication systems.
% Despite these challenges, research and development in THz communication is ongoing, and it is expected that THz communication will play a significant role in the future of wireless communication.

% However, there are also some challenges associated with using the THz frequency band for communication. One of the main challenges is the high absorption of THz waves by water vapor and other atmospheric gases, which can limit the range of THz communication systems. In addition, the high cost and complexity of THz hardware has been a barrier to the widespread adoption of THz communication systems.



% \begin{itemize}
%     \item Explain short-range micro-scale applications and give examples that conducted measurements in that direction.
%     \item Our measurement setup and configurations match with micro-scale communication applications.
%     \item ...
% \end{itemize}

% Throughout the paper, a lowercase bold letter ${\mathbf{x}}$ denotes a vector, and an uppercase bold letter $\mathbf{X}$ denotes a matrix. The probability density function of the uniform distribution is represented as $\mathcal{U}$.
% $\mathcal{F}_{\operatorname{x}}(\cdot)$ denotes a function of the given subscript x. The superscript ${*}$ in text and figures denotes the sparse representation of the channel.


 % $\mathcal{R}e\{\cdot\}$ represents the real-valued term of the complex baseband signal $r(t)$.
    % is the real part of the complex baseband signal $r(t)$. 
    
% $a_l$ and $t_l$ represents attenuation and delay coefficients for the given $l^{th}$ multipath source. 
 % The corresponding complex baseband representation of the multipath channel impulse response is
    % In the case of only the \ac{los} component, $L=1$ in Eq. \eqref{imp_resp_mult} and \ac{los} channel can be given as



    % The measurements~\cite{txmh-mz22-22} are obtained in an anechoic chamber that only allows LOS propagation. 
% The histogram of the received powers and instantaneous SNR values are modeled with Gamma mixtures.
% with parameters $\alpha_k$ and $\beta_k$ which are the shape and rate parameters of the $k^{th}$ mixture component, respectively. 
% To model the instantaneous SNR values with Gamma mixtures, a parameter estimation algorithm is required. 
% The Gamma mixture was chosen for this study because it has traceable CDF and MGF. Thus, it can provide an approximation for fading channels~\cite{atapattu2011mixture}.
% Furthermore, by adjusting its parameters, a wide range of distributions can be represented with high accuracy, and as shown in \cite{wiper2001mixtures}, any arbitrary PDFs on $(0, \infty)$ can be modeled using the Gamma mixture.



% It has been demonstrated that any arbitrary probability density function (PDF) on the positive real line  $(0, \infty)$ can be modeled using a mixture of Gamma distributions~\cite{wiper2001mixtures}.
% Furthermore, the Gamma mixture model (GMM) can provide an approximation for fading channels~\cite{atapattu2011mixture} with its traceable CDF and MGF. Thus GMM is used to model the received signal power $P_{rx}$.
% Note that it is essential to precisely extract the parameters of the GMM for the instantaneous SNR histograms in order to represent it analytically.


% Thus we used the Dirichlet process Gamma mixture model (DPGMM) \cite{9852427} to find the required clusters underneath the $P_{rx}$ observations and corresponding distribution parameters to these clusters. The analytical GMM PDFs are constructed with the parameters which are extracted by DPGMM, and it is shown in Fig. \ref{fig:estimates} for different settings. 

% One of the main application of the EM is maximum likelihood estimation, where the EM algorithm is used to find the maximum likelihood estimates of parameters in statistical models with latent variables.


% Then, using the measurement data and membership coefficients derived in the E-step, new parameter values $\alpha$, $\beta$, and $\pi$  in the mixture model can be obtained for each Gamma component by updating the equations in the M-step as follows 



% As an error metric, we employed Kolmogorov-Smirnov (KS) test.
% It is a non-parametric method used to compare the distribution of a sample data set to a reference probability distribution. It measures the maximum distance between the sample $F_n(x)$ and the reference $F(x)$ cumulative distribution  functions as given 
% \begin{equation}
%     D_{\mathcal{KS}}(n)=\sup_x\left|F_n(x)-F(x)\right|
% \end{equation}
% where $\sup_x$ denotes the supremum of the set of distances.


% The smaller the p-value, the stronger the evidence that the two samples are from different distributions.


% In addition, there is a mechanism on the platforms that allows precise angle adjustment at 1$^{\circ}$ intervals.

% The measurements utilized in this paper were obtained at the Turkish Science Foundation's (T\"UB\.ITAK) anechoic chamber \cite{Millimet77:online}, which are also available at \cite{2jhd-wp15-19}.


% HPBW horn antennas with 24.8 dBi are used at both the transmitter and receiver. 
% Two identical horn antennas with 24.8 dBi gain are connected at both transmitter and receiver.
% The measurement data consist of complex $S_{21}$ parameters that are 



% Each data consist of 4096 points of complex $S_{21}$ parameters spanning the 60 GHz spectrum between 240 and 300 GHz. The spectrum resolution becomes 14.468 MHz with this configuration. Additionally, IF bandwidth is adjusted to 100 Hz for the experiments, enabling an expansion of the observed dynamic range and a reduction of the noise floor.


% Detailed information about measurement setup can be found in \cite{tekbiyik2021modeling}.
    
% Describe the measurement scenarios and steps.
% Also, describe the bandwidth of the measurements and IF properties.

% Analyses are performed in the time and frequency domains during the measurements.
% Time domain analysis is performed by taking the inverse fast Fourier transform (IFFT) of the measurements.


% The EM algorithm is able to pass the KS test for $90\%$ of all settings. This is because EM algorithm converges to the local maxima rather than the global maxima. 
% Also, the EM algorithm does not always guarantee convergence to the local maxima; it only guarantees convergence to a point with zero gradients according to the parameters and depending on the initialization step~\cite{}. 
% As a result, the EM algorithm might occasionally become stuck at the saddle points \cite{}.



% To accurately model the channel capacity and outage probability of the THz band, it is crucial to have a precise representation of the instantaneous SNR. However, this can be a challenge since the THz sub-bands do not always exhibit the same characteristics and can have uneven distribution in terms of received power due to their unique spectral characteristics. Furthermore, the measurements covering the 60 GHz bandwidth may exhibit fluctuations in the received power across the band due to factors such as path loss and molecular absorption. Thus, it's important to have a model that can account for the different forms and variations in the instantaneous SNR across the THz band.

% To determine the communication capabilities of the THz spectrum, it is crucial to have a precise understanding of the instantaneous signal-to-noise ratio (SNR). This can be obtained by modeling the empirical values of the SNR, however this task is complicated by the fact that THz sub-bands have distinct forms and the received power distribution is often not smooth due to their unique spectral properties. Furthermore, the 60 GHz bandwidth covered by the measurements can lead to variations in received power due to factors such as path loss and molecular absorption across the band.

% Since the measurements span the 60 GHz bandwidth and THz sub-bands do not always have the same form and rarely follow a smooth distribution in terms of received power due to their unique spectral characteristics, the instantaneous SNR can not be represented with a single distribution. 


% !!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
% 60 GHz bandın dağılımının karışık olduğunu anlat ve tek bir dağılım ile modelleyenemeyeceğini belirt bu nedenle mixture dağılım seçildi bunu vurgula !
% !!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!




% \begin{figure*}
%     \centering
% \includegraphics[width=0.8\linewidth]{fig/20cm5derece.eps}
%     \caption{PDF of instantaneous SNR at 20 cm $5^{\circ}$ for 60 GHz bandwidth.}
%     \label{fig:experimental_pdf}
% \end{figure*}


% The average channel capacity of a single-input single-output (SISO) channel, the capacity can be evaluated using Shannon's theorem by averaging the instantaneous channel capacity over the SNR distribution as
% \begin{equation}
% C=\int_0^{\infty} B \log _2(1+x) f_\gamma(x) d x.
% \label{eq:capacity_int}
% \end{equation}


% The channel capacity for the measurements can be calculated either by evaluating the Eq. \eqref{eq:capacity_int} numerically with the experimental 
% PDF values or placing the mixture parameters that are extracted with DPGMM to the Eq. \eqref{eq:closed_form_capacity}.


% In this paper, measurements that are collected from 190 different settings spanning 60 GHz bandwidth are analyzed by channel impulse and channel frequency response. The channel model for the micro-scale communication systems operating between 240 GHz-300 GHz is investigated by utilizing Gamma mixtures. To extract the mixture parameters, the EM algorithm and DPGMM are employed, and the suitability of the GMM is validated with the KS test. 
% By using the GMM parameters, the average channel capacity is evaluated for all 190 different settings to see the effect of the distance and misalignment.



% \author{\IEEEauthorblockN{Erhan Karakoca\IEEEauthorrefmark{1}\IEEEauthorrefmark{3}, Hasan Nayir\IEEEauthorrefmark{1}\IEEEauthorrefmark{3}, Gizem Sümen \IEEEauthorrefmark{1}\IEEEauthorrefmark{3}, Güneş Karabulut Kurt\IEEEauthorrefmark{2}, Ali Görçin\IEEEauthorrefmark{4}}
